Generators for the cohomology of the moduli space of irregular parabolic Higgs bundles

We prove that the pure part of the cohomology ring of the moduli space of irregular $\underline{\xi}$-parabolic Higgs bundles is generated by the K\"{u}nneth components of the Chern classes of a universal bundle and the Chern classes of the successive quotients of a universal flag of subbundles. As an application, in the regular full-flag case, we demonstrate a similar result for the cohomology ring of the moduli spaces of parabolic and strongly parabolic Higgs bundles.

==> Purity.tex <==
\section{Purity}\label{sec:purity}



In this section, we study the purity of $\Q$-mixed Hodge structure on $H^*(\huxi,\Q)$. For simplicity, we write $\mathcal{H}=\relativeh$ and $\mathcal{N}=\nld$. We first state main results. 

\begin{theorem}\label{thm: main full flag}

   When $n=1$ and $\underline{m}$ represents the full flag type, for any $\xi \in \mathcal{N}$, the restriction morphism 
    \[
    \iota_\xi^*:H^*(\mathcal{H},\Q) \to H^*(\huxi,\Q)
    \]
    is an isomorphism of $\Q$-mixed Hodge structures where $\iota_\xi:\huxi \hookrightarrow \mathcal{H}$ is a canonical inclusion. In particular, both are of pure type. 
\end{theorem}



The proof relies on the property of semi-projective varieties

\begin{definition}\cite[Definition 1.1.1]{HauselRodriguez2013}
    Let $X$ be a non-singular quasi-projective variety over $\C$ with a $\C^\ast$-action. We call $X$ semi-projective if the following two conditions hold:
    \begin{enumerate}
        \item the fixed point set $X^{\C^\ast}$ is proper
        \item for every $x \in X$, the limit $\lim_{\lambda \to 0}\lambda x$ exists for $\lambda \in \C^\ast$.
    \end{enumerate}
\end{definition}

\begin{prop}\label{prop:semiprojHausel}\cite[Corollary 1.3.3]{HauselRodriguez2013}
    Let $X$ be a non-singular complex algebraic variety and $f:X \to \C$ is a smooth morphism. Also, suppose that $X$ is semi-projective with a $\C^\ast$-action making $f$ equivariant covering a linear action of $\C^\ast$ on $\C$ with positive weight. Then the fibers $X_c:=f^{-1}(c)$ have isomorphic cohomology supporting pure mixed Hodge structures. 
\end{prop}

\begin{lem}
    When $n=1$ and $\underline{m}$ represents the full flag, the relative moduli space $\mathcal{H}$ is semi-projective.
\end{lem}
\begin{proof}
First, note that we have a natural scaling $\C^\ast$-action on $\mathcal{H}$: for $t \in \C^\ast$, $(E, E_D^\bullet, \alpha, \Phi) \in \mathcal{H}$, the action is defined as $t\cdot (E, E_D^\bullet, \alpha, \Phi):=(E, E_D^\bullet, \alpha, t\Phi)$. Similarly, there is a scaling $\C^\ast$-action on $M$ such that the isomorphism $\mathcal{H} \cong M$ we showed in Proposition \ref{prop:isomodulispace} is compatible with these scaling $\C^\ast$-actions. The conclusion follows from the \cite[Corollary 5.12] {Yokogawa-compactification} which shows that $M$ is semi-projective with respect to the scaling $\C^\ast$-action. 
\end{proof}



\begin{proof}[Proof of Theorem \ref{thm: main full flag}]
By iteratively applying Proposition \ref{prop:semiprojHausel} to the canonical morphism $P:\mathcal{H} \to \mathcal{N}$, we achieve the purity of the $\Q$-mixed Hodge structure on $H^*(\huxi)$ for any $\xi\in \mathcal{N}$. Since $P$ is smooth, the pullback morphism 
\[
\iota_\xi^*:H^*(\mathcal{H}) \to H^*(\huxi)
\]
induced by the canonical inclusion $\iota_\xi:\huxi \hookrightarrow\mathcal{H}$ is an isomorphism of $\Q$-mixed Hodge structures. This completes the proof. 
\end{proof}

\todo{cite Komyo somewhere?}

Following from Theorem \ref{thm:purgen}, we have generation results for the regular full flag case. $M

\begin{cor}
    The cohomology of the coarse moduli space of parabolic (resp. strongly parabolic) Higgs bundles $M$ (resp. $M^s$) is generated by the Künneth components of the Chern classes of the universal bundle $\mathcal{E}$ and the universal flag bundles $Q^i$. 
\end{cor}

Let $\m E$ be the universal bundle on $\m H\times C$ and $\m E_{\uxi}$ be the universal bundle on $\huxi\times C$. Let $\m E^\bullet_{\m H\times p}$ and $\m E^\bullet_{\huxi\times p}$ be the universal flag subbundles on $\m H\times p$ and $\huxi\times p$, respectively. Let $Q^i:=\m E^i_{\m H\times p}/\m E^{i-1}_{\m H\times p}$ and $Q^i_\uxi:=\m E^i_{\huxi\times p}/\m E^{i-1}_{\huxi\times p}$ be their associated quotients respectively. Clearly, $(\iota_\uxi\times \Id)^*\m E = \m E_\uxi$ and $\iota_\uxi^*\m E^\bullet_{\m H\times p} = \m E^\bullet_{\huxi\times p}$.  We also see that $Q^i_\uxi$ is isomorphic to $\iota_\uxi^*Q^i$. It is easy to see that the left-hand K\"{u}nneth components of the Chern classes of $\m E_\uxi$ in $H^*(\huxi)$ are exactly the pullback of the left hand K\"{u}nneth components of the Chern classes of $\m E$ in $H^*(\m H)$ along $\iota_\uxi\times \Id$. Moreover, we have $\iota_\uxi^*\ch(Q^i) = \ch(\iota_\uxi^*Q^i_\uxi).$ Since $\iota_\uxi^*: H^*(\m H)\to H^*(\huxi)$ is an isomorphism, it follows from the generation result of $H^*(\huxi)$ that $H^*(\m H)$ is also generated by the K\"{u}nneth components of the Chern classes of $\m E$ and the Chern classes of $\ch(Q^i)$.

We conclude this section by explaining why the same method is not applicable to study the purity when $n>1$. The issue is that $\mathcal{H}$ is not semi-projective because the locus of fixed point $\mathcal{H}^{\C^\ast}$ may not be proper: consider the canonical inclusion $\mathcal{H} \hookrightarrow M\times \mathcal{N}$. Composing with the projection $M \times \mathcal{N} \to M$, we have the finite morphism $\mathcal{H} \hookrightarrow M\times \mathcal{N}$ that is $\C^\ast$-equivariant. Also, since the scaling $\C^\ast$-action is equivariant with respects to the Hitchin morphism $h:M \to B$, the fixed locus belongs to $\mathcal{H}_{\underline{0}} \cap h^{-1}(0)$. While $h^{-1}(0)$ is proper, the restriction $\mathcal{H}_{\underline{0}} \cap h^{-1}(0)$ is in general open. This is because, the freeness condition on the quotient of the flag $E_D^\bullet)$ is in general an open condition. For example, take $D=3p$, $\underline{m}=(3,3)$ and $E$ is a trivial bundle of rank $2$. The restriction $E_D$ is a free $k[t]/t^3$-module of rank 2, $k[t]/t^3\oplus k[t]/t^3$. Let $\Phi$ be a Higgs field whose local form at $D$ is
\[
\Phi|_D=\begin{bmatrix}
    0 & t \\
    0 & 0
\end{bmatrix}
\]
Choose a filtration $0 \subset E_D^1 \subset E_D$ where $E_D^1=(t^2)\oplus (t)$. This filtration is preserved by $\Phi$ while the quotient $E_D/E_D^1$ is not free. 

\begin{conj}
    When $n>1$, the $\Q$-mixed Hodge structure on $H^*(\mathcal{H}_\xi)$ is of pure type for any $\xi \in \mathcal{N}^\circ$. 
\end{conj}

\SJ{}
\SJ{After this point, do you want to add anything else?}

Two questions. Assume the full-flag case

\begin{itemize}
    \item As explained above, $h^{-1}(0) \cap \mathcal{H}$ is not proper in general. We say a bit more about the structure of $h^{-1}(0)$. It seems like there exists an algebraic stratification 
    \[
    \cdots \subset H_l \subset \cdots \subset H_1 \subset h^{-1}(0) 
    \]
    where $H_1=\mathcal{H} \cap h^{-1}(0)$. For $(E,\Phi) \in h^{-1}(0)$, we may stratify it based on the locally freeness condition on the successive quotient. In other words, the number of locally free successive quotient would induce a stratification on $h^{-1}(0)$. 
    \item Can we stratify our moduli spaces in terms of the rank of the flag? 
    \item Let $\mathcal{H}_{\mathbb{A}^1} \to \mathbb{A}^1$ be an one-parameter family with a generic $\xi \in \mathbb{A}^1$. I am wondering how the induced Hitchin fibration on $\mathcal{H}_{\mathbb{A}^1}$. Let's ignore the ordering for now. The Hitchin map $\mathcal{H}_{\mathbb{A}^1} \to \mathbb{A}^1 \times B_0$ has closed fibers over $(\xi,b)$ with $\xi \neq 0$ since the freeness condition is vacuous. It is not clear that a fiber over $(0,b)$ is closed. 

    If this picture is right, how about taking the relative closure of $\mathcal{H}_{\mathbb{A}^1}|_{\mathbb{A}^1\setminus 0}$ inside $M$. Can we make a moduli interpretation of $\overline{\mathcal{H}_{\mathbb{A}^1}|_{\mathbb{A}^1\setminus 0}} \cap h^{-1}(0)$? The reason that I am thinking about this is the moduli of strongly parabolic Higgs bundles with the freeness condition is not necessarily pure (Also, this may not be needed to prove the purity for $\huxi$). So, the idea is to characterize the smaller one, which has closed fibers with respects to $h$, and show that it is smooth/mildly singular. Actually, we don't need to take the restriction over $\mathbb{A}^1$, rather work with $\mathcal{N}^\circ$ consisting of generic $\xi$. 

    Relation to the previous question, if we were to construct a sequence $(E_a, E_{D,a}, \Phi_a) \in \mathcal{H}|_{\mathcal{N}^\circ}$ that converges to $(E,E_D^\bullet, \Phi)$ with $E_D^\bullet$ not obeying freeness condition, there is a jump of the rank of the quotient in $E^i_{D,a}/E_{D,a}^{i+1}$ for some $i$ at $a=0$. E.g. Is this allowable for our numerical conditions?
\end{itemize}

